Categories of Nets

We present a unified framework for Petri nets and various variants, such as pre-nets and Kock's whole-grain Petri nets. Our framework is based on a less well-studied notion that we call $\Sigma$-nets, which allow finer control over whether tokens are treated using the collective or individual token philosophy. We describe three forms of execution semantics in which pre-nets generate strict monoidal categories, $\Sigma$-nets (including whole-grain Petri nets) generate symmetric strict monoidal categories, and Petri nets generate commutative monoidal categories, all by left adjoint functors. We also construct adjunctions relating these categories of nets to each other, in particular showing that all kinds of net can be embedded in the unifying category of $\Sigma$-nets, in a way that commutes coherently with their execution semantics.

==> Presentation/macros.tex <==
% -*- mode: latex; TeX-master: "paper.tex" -*-

%% Math definitions

\newcommand{\defin}[1]{{\bf \boldmath{#1}}}

\newcommand{\id}[1]{\mathrm{Id}_{#1}}
\newcommand{\op}{^\mathrm{op}}
\newcommand{\PN}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\N}{\mathbb{N}}
\newcommand{\SigmaNet}{\ensuremath{\Sigma\text{-net}}\xspace}

% Category Names
\newcommand{\CatDef}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\Fin}{\CatDef{Fin}}
\newcommand{\Set}{\CatDef{Set}}
\newcommand{\SSMC}{\CatDef{SSMC}}
\newcommand{\StrMC}{\CatDef{StrMC}}
\newcommand{\CMC}{\CatDef{CMC}}
\newcommand{\PreNet}{\CatDef{PreNet}}
\newcommand{\SigmaNetCat}{\CatDef{\Sigma{\text{-}net}}}
\newcommand{\Petri}{\CatDef{Petri}}
\newcommand{\WGPet}{\CatDef{WGPet}}
\newcommand{\Cat}{\CatDef{Cat}}
\newcommand{\CommDuoid}{\CatDef{CommDuoid}}
\newcommand{\PROP}{\CatDef{PROP}}
\newcommand{\Open}{\mathbb{O}\mathbf{pen}}
\newcommand{\pre}{\mathrm{pre}}
\newcommand{\pet}{\mathrm{pet}}
\newcommand{\A}{\CatDef{A}}
\newcommand{\B}{\CatDef{B}}
\newcommand{\X}{\CatDef{X}}
\newcommand{\C}{\CatDef{C}}
\newcommand{\D}{\CatDef{D}}
\newcommand{\E}{\CatDef{E}}
\newcommand{\Comma}[2]{(#1\downarrow #2)}

\newcommand{\maps}{\colon}
\newcommand{\simrightarrow}{\xrightarrow{\raisebox{-3pt}[0pt][0pt]{\ensuremath{\sim}}}}
\newcommand{\simRightarrow}{\xRightarrow{\raisebox{-3pt}[0pt][0pt]{\ensuremath{\sim}}}}
\newcommand\NEarrow{\mathrel{\rotatebox[origin=c]{45}{$\Rightarrow$}}}
\newcommand\Narrow{\mathrel{\rotatebox[origin=c]{90}{$\Rightarrow$}}}

%% Environments
\newtheorem{thm}{Theorem}[section]
\crefname{thm}{Theorem}{Theorems}
\newaliascnt{prop}{thm}
\newtheorem{prop}[prop]{Proposition}
\aliascntresetthe{prop}
\crefname{prop}{Proposition}{Propositions}
\newaliascnt{lem}{thm}
\newtheorem{lem}[lem]{Lemma}
\aliascntresetthe{lem}
\crefname{lem}{Lemma}{Lemmas}
\theoremstyle{definition}
\newaliascnt{defn}{thm}
\newtheorem{defn}[defn]{Definition}
\aliascntresetthe{defn}
\crefname{defn}{Definition}{Definitions}
\theoremstyle{remark}
\newaliascnt{ex}{thm}
\newtheorem{ex}[ex]{Example}
\aliascntresetthe{ex}
\crefname{ex}{Example}{Examples}
\newaliascnt{rmk}{thm}
\newtheorem{rmk}[rmk]{Remark}
\aliascntresetthe{rmk}
\crefname{rmk}{Remark}{Remarks}

\crefformat{section}{Section~#2#1#3}


% TikZ

\tikzstyle{simple}=[-,line width=2.000]
\tikzstyle{arrow}=[-,postaction={decorate},decoration={markings,mark=at position .5 with {\arrow{>}}},line width=1.100]
\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{edgelayer,nodelayer,main}

\tikzstyle{none}=[inner sep=0pt]

%\definecolor{lblue}{rgb}{0,250,255}

% Place style
\tikzstyle{place}=
[circle,thick,draw=blue!75,fill=blue!20,minimum size=6mm]

% Transition style
\tikzstyle{transition}=
[rectangle,thick,draw=black!75,fill=black!20,minimum width=1mm, minimum height=4mm]

% This controls the 3d POV for sigma-nets
\def\xcoord{-1.2}
\def\ycoord{0.5}

% sigma-net tank colour and opacity
\def\transitionbgrd{gray!50}
\def\transitionop{0.3}

%\tikzstyle{species}=[circle,fill=yellow,draw=black,scale=1.15]
%\tikzstyle{transition}=[rectangle,fill=lblue,draw=black,scale=1.15]
\tikzstyle{inarrow}=[->, >=stealth, shorten >=.03cm,line width=1.5]
\tikzstyle{empty}=[circle,fill=none, draw=none]
\tikzstyle{inputdot}=[circle,fill=purple,draw=purple, scale=.25]
\tikzstyle{inputarrow}=[->,draw=purple, shorten >=.05cm]
\tikzstyle{simple}=[-,draw=purple,line width=1.000]

%% EXTENSIBLE SLASHED ARROWS
% Making extensible slashed arrows, by modifying the underlying AMS code.
% Arguments are:
% 1 = arrowhead on the left (\relbar or \Relbar if none)
% 2 = fill character (usually \relbar or \Relbar)
% 3 = slash character (such as \mapstochar or \Mapstochar)
% 4 = arrowhead on the left (\relbar or \Relbar if none)
% 5 = display mode (\displaystyle etc)
\makeatletter
\def\slashedarrowfill@#1#2#3#4#5{%
  $\m@th\thickmuskip0mu\medmuskip\thickmuskip\thinmuskip\thickmuskip
   \relax#5#1\mkern-7mu%
   \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
   \mathclap{#3}\mathclap{#2}%
   \cleaders\hbox{$#5\mkern-2mu#2\mkern-2mu$}\hfill
   \mkern-7mu#4$%
}
\def\rightslashedarrowfill@{%
  \slashedarrowfill@\relbar\relbar\mapstochar\rightarrow}
\newcommand{\xslashedrightarrow}[2][]{%
  \ext@arrow 0055{\rightslashedarrowfill@}{#1}{#2}}
\newcommand{\profto}{\xslashedrightarrow{}}
\let\xprofto\xslashedrightarrow

% Personal fixme commands
\FXRegisterAuthor{ms}{anms}{Mike}
\FXRegisterAuthor{jb}{anjb}{John}
\FXRegisterAuthor{jm}{anjm}{Jade}
\FXRegisterAuthor{fg}{anfg}{Fab}


==> Presentation/packages.tex <==
% -*- mode: latex; TeX-master: "paper.tex" -*-

\usepackage{amsmath,amsthm,amsfonts}
\usepackage[utf8]{inputenc}
\usepackage{tikz-cd}
\usepackage{xspace}
\usepackage[all,cmtip]{xy}
\usepackage{mathtools}
\usepackage{color}
\definecolor{myurlcolor}{rgb}{0.3,0,0}
\definecolor{mycitecolor}{rgb}{0,0,0.8}
\definecolor{myrefcolor}{rgb}{0,0,0.8}

\usepackage{tikz}
\usepackage{tikz-cd}
  \usetikzlibrary{backgrounds,circuits,circuits.ee.IEC,shapes,petri,fit,matrix}
\usepackage{adjustbox} % needed to rescale tikz-cd images

\usepackage[status=draft,mode=multiuser]{fixme}
\fxusetheme{colorsig}

\usepackage{cleveref,aliascnt}



==> sections/sigmaNet.tex <==
\scalebox{0.8}{
\begin{tikzpicture}
% Base net & tank bottom
  \begin{scope}[
      yshift=0,every node/.append style={
      yslant=\ycoord,xslant=\xcoord},yslant=\ycoord,xslant=\xcoord
      ]
    \begin{pgfonlayer}{nodelayer}
      \node [place,tokens=0] (1a) at (-2,0.75) {};
      \node [place,tokens=0] (1b) at (-2,-0.75) {};      			
      \node [place,tokens=0] (3a) at (2,0) {};
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
      \draw[style=inarrow, thick] (1a) to  (-0.5,0.75);
      \draw[style=inarrow, thick] (1b) to  (-0.5,-0.75);
      \draw[style=inarrow, thick] (0.5,0) to (3a);
    \end{pgfonlayer}
    
    % Tank bottom
      \fill[\transitionbgrd, opacity=\transitionop]  (-0.5,-1) rectangle (0.5,1);
      \node (11) at (-0.5,1) {};
      \node (21) at (-0.5,-1) {};
      \node (31) at (0.5,-1) {};
      \node (41) at (0.5,1) {};
  \end{scope}

% First transition
  \begin{scope}[
      yshift=8,every node/.append style={
      yslant=\ycoord,xslant=\xcoord},yslant=\ycoord,xslant=\xcoord
      ]
    \begin{pgfonlayer}{nodelayer}
      \node [transition] (2b) []  at (0,0) {};  
    \end{pgfonlayer}
    \begin{pgfonlayer}{edgelayer}
      \draw[thick, in=135, out=-45] (-0.5,0.5) to  (2b);
      \draw[thick,  in=225, out=45] (-0.5,-0.5) to  (2b);
      \draw[thick] (2b) to  (0.5,0);
    \end{pgfonlayer}
  \end{scope}

% Second transition
  \begin{scope}[
      yshift=22,every node/.append style={
      yslant=\ycoord,xslant=\xcoord},yslant=\ycoord,xslant=\xcoord
      ]
    \begin{pgfonlayer}{nodelayer}
      \node [transition] (2b) []  at (0,0) {};  
    \end{pgfonlayer} 
    \begin{pgfonlayer}{edgelayer}
      \draw[thick, in=225, out=-45] (-0.5,0.5) to  (2b);
      \draw[thick,  in=135, out=45] (-0.5,-0.5) to  (2b);
      \draw[thick] (2b) to  (0.5,0);
    \end{pgfonlayer}
  \end{scope}

% Tank top
  \begin{scope}[
      yshift=30,every node/.append style={
      yslant=\ycoord,xslant=\xcoord},yslant=\ycoord,xslant=\xcoord
      ]

      \fill[\transitionbgrd, opacity=\transitionop]  (-0.5,-1) rectangle (0.5,1);
      \node (14) at (-0.5,1) {};
      \node (24) at (-0.5,-1) {};
      \node (34) at (0.5,-1) {};
      \node (44) at (0.5,1) {};
  \end{scope}

% Tank contours
    \fill[\transitionbgrd, opacity=\transitionop]   (11.center) -- (14.center) -- (24.center) -- (21.center) -- (11.center);
    \fill[\transitionbgrd, opacity=\transitionop]   (21.center) -- (24.center) -- (34.center) -- (31.center) -- (21.center);
    \fill[\transitionbgrd, opacity=\transitionop]   (31.center) -- (34.center) -- (44.center) -- (41.center) -- (31.center);
    \fill[\transitionbgrd, opacity=\transitionop]   (41.center) -- (44.center) -- (14.center) -- (11.center) -- (41.center);

\end{tikzpicture}
}
